REFFLY: Melody-Constrained Lyrics Editing Model

Automatic melody-to-lyric (M2L) generation aims to create lyrics that align with a given melody. While most previous approaches generate lyrics from scratch, revision, editing plain text draft to fit it into the melody, offers a much more flexible and practical alternative. This enables broad applications, such as generating lyrics from flexible inputs (keywords, themes, or full text that needs refining to be singable), song translation (preserving meaning across languages while keeping the melody intact), or style transfer (adapting lyrics to different genres). This paper introduces REFFLY (REvision Framework For LYrics), the first revision framework for editing and generating melody-aligned lyrics. We train the lyric revision module using our curated synthesized melody-aligned lyrics dataset, enabling it to transform plain text into lyrics that align with a given melody. To further enhance the revision ability, we propose training-free heuristics aimed at preserving both semantic meaning and musical consistency throughout the editing process. Experimental results demonstrate the effectiveness of REFFLY across various tasks (e.g. lyrics generation, song translation), showing that our model outperforms strong baselines, including Lyra (Tian et al., 2023) and GPT-4, by 25% in both musicality and text quality.

==> content/dataset.tex <==
\section{Dataset}
% To the best of our knowledge,we are the first to consider the important notes in a melody and the relationship between important notes and words. Thus, we constructed 1, a finetune dataset for lyric revision that does not rely on aligned melody-lyric data, and 2, an expert-annotated validation dataset to evaluate the accuracy of our important note extraction accuracy. \yufei{The 2nd dataset should already have been introduced in your music theories. So just a brief recap letting readers know you used the expert annotated data that has been introduced in section xxx will be good enough.}
\subsection{Training dataset}
The purpose of our training dataset is to teach the model to revise lyrics drafts based on music constraints.
% In order to achieve this, we constructed a finetune dataset that contains the lyrics draft, the music constraint, and the corresponding revised lyrics. 
The source of our finetune dataset are 3500 songs scraped from the internet[]. Using Sudo-Music-Constraint-Generation introduced in section 3.3, we can generate music constraint for each line of the lyric without its melody, alleviating the scarcity and the copyright issue of the aligned data.

% We designed an alignment algorithm to create sudo-music-constraint from pure lyrics, allowing us not requiring aligned melody-lyric data, which is limited in the real world due to copy right issue[].\yufei{Again, put the following alignment algorithm to the previous section. And just co-refer here. By co-refer I mean you should say something like we use the alignment algorithm introduced in xxx to do yyy. You can also have a one-sentence summary to refresh readers' memory.}

% The alignment algorithm assumes the stressed phenom of important words are always corresponds to important note. We define important word as noun and verbs, because nouns typically denote key entities in a text \yufei{need citation to support this reason}, while verbs are essential for capturing the actions or main activities discussed [RAKE]  \yufei{need citation to support this reason}. The alignment algorithm is defined as follow:\\
% Suppose a sentence has k words [$w_1,w_2,...,w_k$] with n syllables [$i_1,i_2,...,i_n$]. 
% \begin{equation}
% i_j = 
% \begin{cases} 
% 1 & \text{if it is a stressed phenom}\\
% 0 & \text{, otherwise}
% \end{cases}
% \end{equation}
% for $j \in [1,n]$.\\
% Then, we can define Music constraint [$m_1,m_1,...,m_n$], such that
% \begin{equation}
% m_j = 
% \begin{cases} 
% 1 & \text{if } i_j = 1 \text{ and } w_z \text{ is noun or verb}\\
% 0 & \text{, otherwise}
% \end{cases}
% \end{equation}
% where $j \in [1,n]$, and $w_z$ is the word corresponding to syllable $i_j$.\\
% With this algorithm, for each original sentence in our song corpus, we generate a corresponding music constraint for it. 
% \yufei{This whole paragraph only explains what you did. But what's more important is why did you do this? Why choose this algorithm? How is this alignment better than Lyra's alignment? Need citations and numbers/comparisons to your claim.}

After getting the music constraint for each line of lyrics, ChatGPT-3.5 is used to rephrase each sentence. In order to make the revised sentence coherent with its context, previous lyrics are included in the input. Accordingly, the input of our finetune dataset is the rephrased sentence, title, music constraint, previous original lyrics, and Chain-of-thoughts reasoning. The output is the original lyrics and some explanation.
In the Chain-of-thoughts reasoning, we provide information about 1, the phenom of each word, 2, number of syllables in original and rephrased sentence, and 3, some guidelines of way to modify the lyric drafts (e.g. make the sentence shorter/longer). The phonetic information is retrieved from the CMU pronounciation dictionary (Weide et al., 1998)\\
\label{sec:appendix}
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/Example_finetune.png}\yufei{Don't use png format for figures, when there are texts. Use pdf instead.}
  \caption{Exemplary data point in the finetune dataset}\yufei{Expand the caption a bit -- readers should be able to understand the figure with captions only, without reading the main texts.}
\label{fig:example}
\end{figure}
\subsection{Validation dataset}
In order to test the accuracy of the important note extraction algorithm, we constructed a 100-songs-dataset that is annotated by professional musicians, highlighting all the important notes in the melody. The music style of this dataset across Jazz, Country, Blues, Folk, Pop, and Comedy.\yufei{This is not clear. I would suggest showing an example while you first introduce this concept in the previous section.}
\subsection{Human evaluation setup}
\textbf{Qualification task} is conducted to select 100 annotators with 1) adequate expertise in song and lyric annotation, and 2) reliable focus on the Mechanical Turk platform. The qualification involved two segments. To evaluate the Turkers' expertise in the field, we designed a task that included the initial verse from 5 different songs, each with ground-truth labels. These songs were chosen with care to avoid unclear cases, allowing for a clear assessment of quality. The selected songs were those whose scores showed a strong correlation with the ground-truth labels.  \songyan{at here can we also follow Lyra's pipeline to rule out irresponsible workers?}\\
\textbf{Annotation Task} 
Our annotation process is relative, with annotators evaluating groups of songs produced by different systems that share the same melody and title. All baseline models were assessed. At least three workers annotated each song, rating the lyrics' quality on a 1-5 Likert scale across five categories related to musicality and text quality. For musicality, the workers rated \textbf{emphasis alignment} (whether the important words were exaggerated in the melody) and \textbf{singability} (whether the melody's rhythm synchronized with the lyrics' rhythm). Regarding text quality, they assessed \textbf{coherence} and \textbf{creativeness}. Lastly, we asked the annotators to rate how much they enjoyed each song \textbf{overall}.

==> old/03-method.tex <==
\section{Lyric Generation Framework}
% why we have revision model, input output/why we need it, how having these input/output make the model unique
In order to generate emphasis-aligned, singable, and coherent lyrics, and being suitable of more downstream tasks (e.g. lyric translation or generating lyrics adhere to song structure), we propose a lyric revision framework: it uses lyrics-only data during training and guided by music constraints extracted from the melody during inference.
% \yufei{The current version is a bit messy and need significant rewriting. For EVERY paragraph in this section, can I request you to write their functions in 5-10 words, in the beginning of each paragraph.}


% \subsection{Important-Notes-Extractor}\yufei{this part is somewhat redundant. I would remove.}
% In order to catch the importance of a note, we consider the time signature, syncopation, and pitch jump.\\
% A note is defined as important if any one of the following condition is satisfied: 1, it is in an stressed beat determined by time signature; 2, it is a syncopation; or 3, it is a big pitch jump.\\
% Big pitch jump means the difference of pitch values between two consecutive note is larger than the average pitch difference in the melody. For more details please refer to the important note extractor section in appendix

\subsection{Revision model}
\label{sec:revision_model}
\songyan{briefly talks about motivation of doing revision}

% For a more broaden applicability of the LLM-enhanced lyric writing, we propose the first revision-based lyrics generation model that generates high-quality lyrics, which fits the given melody, while keep the meaning of provided lyrics draft unchanged. Our model can not only generate a lyrics for a whole song, but also being capable of other downstream tasks like lyric translation.\\

To broaden the applicability of LLM-enhanced lyric writing, we introduce the first revision-based lyric generation model. This model produces high-quality lyrics that fit a given melody while preserving the meaning of the provided lyric draft. Moreover, our model is versatile, capable of generating lyrics for an entire song and performing additional downstream tasks such as lyric translation.

\songyan {Our method to fulfill syllable planning and emphasize-alignment}

% In order to generate high-quality lyrics that is singable and emphasized-aligned, we need to solve the syllable planning task (generate a self-contained sentence with desired number of syllables), and map the important words to important notes in the same time. This mapping aims to align all important words to prominent note, but not all prominent notes to important words. Previous work \cite{tian2023unsupervised} uses constraint decoding to tackle a similar tasks combination -- a syllable planning task with stress-duration mapping (maps longer notes to stressed syllable and vice versa). This stress-duration mapping is a bijective mapping, so it is beneficial to use a constraint decoding algorithm that adds additional weights to those words satisfying the stress-duration alignment when model generate a token for a longer note. Since our mapping is not bijective, we cannot naively adopt a constraint decoding inference scheme. Alternatively, during training, for each sentence, we create a "pseudo music constraint" that has the same format as a real music constraint (shown in Figure ~\ref{fig:example}) So, our model learns to generate emphasize-aligned and singable lyrics based on psuedo music constraint during training, and can follow the real music constraint extracted from the melody during inference. More details about generating pseudo music constraint can be found in Section ~\ref{sec:training_dataset}.

To accomplish this goal, we address two key tasks: syllable planning (creating self-contained sentences with a specified number of syllables) and mapping important words to prominent notes. This mapping specifically aligns all important words with prominent notes, though not every prominent note is matched to an important word. Prior work \cite{tian2023unsupervised} tackles a similar combination of tasks—syllable planning alongside stress-duration mapping, which aligns longer notes with stressed syllables and vice versa. This stress-duration mapping is bijective, allowing the use of constraint decoding algorithms that assign additional weight to words that meet the stress-duration alignment when the model generates a token for a longer note.

Since our mapping strategy is not bijective, adopting a straightforward constraint decoding approach is not feasible. Instead, during training, we create a "pseudo music constraint" for each sentence, formatted similarly to an actual music constraint (as illustrated in Figure ~\ref{fig
}). This approach enables our model to learn how to produce lyrics that are emphasis-aligned and singable based on pseudo music constraints. During inference, the model applies real music constraints extracted from the melody. Further details on generating pseudo music constraints are discussed in Section ~\ref{sec
}.

 \songyan {Our method for coherence, introduce CoT}

Coherence is also important for high-quality lyrics. We achieve this by providing previous generated lyrics and title for each every lyrics draft in training, so that the model can adhere to these information during inference. To further boost the performance, we designed Chain-of-Thoughts prompt\cite{wei2022chain} for each training data points. We show the effectiveness of these prompts in Section ~\ref{sec:ablation}. For more details about the prompts, please refer to the appendix.

\subsection{Song Structure}
\songyan { why it is important, how to add that into the training process}\\
\songyan{I want to make this subsection longer, so I include information about the input/output, and training llama at here. I'm not sure if i can do this or not since they seems to belong to 4.1}

Most popular songs have paragraph-by-paragraph structure, such as verse-bridge-chorus\cite{watanabe-goto-2020-lyrics}. However, this important aspect in lyric generation has been overlooked in previous works. We add the song structure information to the training process and the Chain-of-thought prompt, so that the model learns to generate lyrics follow the provided song structure. Considering all the above-mentioned information, we finetune LLaMA-13b\cite{Touvron2023update} as our revision model.  

\songyan {finally talks about the input and output}

The input of our revision model is 1, lyrics drafts, 2, music constraints, 3, previously generated lyrics, 4, title, 5, song structure; and the output is 1, the generated lyrics and 2, some explainable verification. This process is illustrated in Figure ~\ref{fig:overview} 

% We introduce our lyrics-only training dataset construction process. We then present the input and output of the revision model.\\
% In addition to ensure singability and emphasize-alignment, our model generates lyrics that adhere to specific \textbf{song structures} (e.g. verses or choruses), and maintains coherence throughout the song. We achieve this by providing song structure, previous generated lyrics, and title for each training data points, so that the model can adhere to these information during inference. To further boost the performance, we designed Chain-of-Thoughts prompt\cite{wei2022chain} for each training data points. We show the effectiveness of these prompts in Section [ablation]. For more details about the prompts, please refer to the appendix.

% With all the above-mentioned elements, we construct the training dataset and use it to finetune LLaMA-13b\cite{Touvron2023update}. To construct the training dataset, for each sentence in our data source (which are some real songs), we generate a pseudo constraint using pseudo-music-constraint-generation algorithm; then, we use ChatGPT-3.5 to rephrase this sentence as the lyric draft. With all the aforementioned elements, the model learns to reconstruct the real songs. The training data construction process is illustrated in Figure \ref{fig:??}. 

% Finally, the input of the model is 1, lyrics drafts, 2, music constraints, 3, previously generated lyrics, 4, title, 5, song structure; and the output is 1, the generated lyrics and 2, some explainable verification. 


% As illustrated in Figure ?, The input of our revision model takes in the a sentence of the lyric draft and a musical phrase in the melody, and generate the revised lyric that it is aligned with the musical phrase. In order to align the lyric to the melody, the generate lyric should be singable, intelligence, and coherent. This means that 1, one note in melody should correspond to zero or one syllable; 2, important words should be mapped to important notes; and 3, the generate sentence should be coherent with previously generated sentences.\\

% We finetune LLaMA 13b to fulfill the above-mentioned considerations. As is shown in Figure  \ref{figxxx}, with number of desired syllables, lyric drafts, music constraints, previously generated lyrics, and some Chain-of-Thoughts prompts, the model learns to generate lyrics that aligns with the music constraint and is coherent with previously generated lyrics. 




% There is one more challenge: finetuning a model to achieve aforementioned tasks requires large amount of aligned score-lyrics data, because  the lyrics and their corresponding music constraint is needed. However, there are not many such aligned data available, and often have copyright issues []. To alleviate this challenge, we proposed a Sudo-Music-Constraint-Generation algorithm that can generate a music constraint from pure lyrics without its score.\\
% The \textbf{Sudo-Music-Constraint-Generation} algorithm assumes the stressed phenom of important words are always corresponds to important note and each syllable corresponds to one notes. We define important word as noun and verbs, introduced in Section 2.3 (\yufei{don't just write the number, use reference}. From these two assumptions, the algorithm generate a list of special tokens representing important and unimportant notes, where the notes corresponding to important words are important, others are unimportant. More detailed explanation can be found in the appendix.\yufei{The above two sections are really unclear to me. Please use illustration. Suggest to move Figure \ref{fig:example} forward.}



% \yufei{The Sudo-Music-Constraint-Generation is not really a methodology, and should go into the dataset section. Also, I don't believe we have space for such a detailed explanation.}
% With this algorithm, we can generate a sudo music constraint for any given sentence, so that we can train our model to map important words to important notes during inference with real music constraints.
% \yufei{This whole paragraph only explains what you did. But what's more important is why did you do this? Why choose this algorithm? How is this alignment better than Lyra's alignment? Need citations and numbers/comparisons to your claim.}
% Challenges\\
% Singable -- one note correspond to zero or 1 syllables\\
%     Solution: \\
%     1, add syllable information\\
%     2, mapping\\
% Intelligence -- important words need to correspond to important notes.\\
%     solution:\\
%     1, Provide the information about music constraint\\
% Revision -- similar to draft sentences\\
%     Solution:
%     Make sure input and output sentence are similar
% Coherence \\
% solution:\\
%     provide previous lyrics


% \subsection{Adding Structure Information}
% What are the adjustments we made to generate full-length songs.

\subsection{Inference}
\songyan{high level idea/motivation of overgen+mapping}

During inference, we use real music constraint extracted from melody using our rule-based \textit{prominent note extractor} introduced in Section ~\ref{sec:prominent_note} to guide the generation. 

To further improve the ability of generating singable and emphasize-aligned lyrics, we proposed an over generate and mapping algorithm, that inspired by the use of \textit{ties}, a widely used musical notation in songwriting. A \textit{tie} serves to map multiple notes to a single syllable.\cite{perricone2018great} We can achieve better emphasize-alignment by adding ties to the melody and won't harm the singability and coherence. \\ 
% \Require Sentence $s$, Music constraint $m$, Maximum number of ties $K$
% \Ensure Singable and emphasize-aligned lyrics

% \State Generate 16 outputs for each input using diverse beam search
% \begin{algorithm}
% \caption{Over Generate and Mapping Algorithm}
% \label{alg:ogm}
% \begin{algorithmic}[1]
% \State Initialize $P \leftarrow []$
% \State $O \leftarrow $ LLM $(input)$
% \While{$P == []$}
%     \For{each output $o$ in $O$}
%         \State $o_{ties}=$ num ties needed $(o,c)$ 
%         \If{ $ 0 \leq o_{ties}  \leq K$}
%             \State $o_{m} =$ possible tie pos$(o,o_{ties},c)$ 
%             \State $o_{best} = $max prosody$(o_{m})$
%         \EndIf
%     \EndFor
%     \If {$P == []$}
%         \State$input =$ get rephrased input $(input)$
%     \EndIf
% \EndWhile

% \State $result$ = most similar to $(input)$
% \end{algorithmic}
% \end{algorithm}



In \textbf{Over generate and mapping} algorithm

, we firstly use diverse beam search [] to generate multiple candidates for each input. Then, we utilize our mapping algorithm to further maximize the alignments with music constraint for each outcome. The final output is chosen as the candidate that 1, is singable, 2, is emphasize-aligned, and 3, preserve the draft meaning the most.\\ 
% We define a lyric being singable if each note corresponds to one or zero syllables, and 2, each syllable in a multi-syllables word corresponds to a note that is no longer than a half-note. \\
For a input sentence $s$ and music constraint $m$, the mapping algorithm can be defined as follows:\\
Step 1: deciding number of ties to add:
\begin{equation}
\#ties = \#notes(m) - \#syllables(s)
\end{equation}
Step 2: Define $K$ as a hyper-parameter indicating the maximum number of ties we allows in each musical phrases.\\
If $\#ties < 0$ or $\#ties > K$, reject this input. Otherwise, try all possible ways to insert ties, returning the one with the maximum number of important words being mapped to the important notes. \\
If the algorithm rejects all the outputs from overgeneration at step 2, the draft sentence is rephrased into a new draft, which would be feed to the model with the same music constraint. \\
If step 2 didn't reject all outputs, apply the mapping algorithm to all of outputs from diverse-beam search, and the final output is the one with maximum number of important words being mapped to the important notes. If there are multiple perfect-matching outputs, the final output is the one that is most similar to the input sentence calculated by BertScore []. \\
An illustrative example is shown in Figure ~\ref{fig:overview} 


% \subsection{Align Important Word with Important Note}
% \textbf{Generating music constraint for pure text}\\
